A generalized framework for direct discontinuous Galerkin methods for nonlinear diffusion equations

In this study, we propose a unified, general framework for the direct discontinuous Galerkin methods. In the new framework, the antiderivative of the nonlinear diffusion matrix is not needed. This allows a simple definition of the numerical flux, which can be used for general diffusion equations with no further modification. We also present the nonlinear stability analyses of the new direct discontinuous Galerkin methods and perform several numerical experiments to evaluate their performance. The numerical tests show that the symmetric and the interface correction versions of the method achieve optimal convergence and are superior to the nonsymmetric version, which demonstrates optimal convergence only for problems with diagonal diffusion matrices but loses order for even degree polynomials with a non-diagonal diffusion matrix. Singular or blow-up solutions are also well captured with the new direct discontinuous Galerkin methods.

==> nonlinear diffusion paper arxiv preprint/shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
%\usepackage[utf8]{inputenc}
%\usepackage[T1]{fontenc}
%\usepackage{amsmath}
%\usepackage{amssymb}
%\usepackage{amsthm}
%\usepackage{mathrsfs}  
\usepackage{graphicx,subcaption}
\usepackage[left=2.2cm,right=2.5cm,top=2.5cm,bottom=3.5cm]{geometry}
%\usepackage[table]{xcolor}
\usepackage{boldline}
%\usepackage{lineno}
\usepackage{tikz}
%\usepackage{authblk}
% fancy jump notations
\usepackage{stmaryrd} 
\usepackage{fancyhdr}
%
\usepackage{titlesec}
\usepackage{secdot}
%
%\usepackage{hyperref}
%\hypersetup{
%    colorlinks=true,
%    linkcolor=blue,
%    citecolor=blue,
%    filecolor=magenta,      
%    urlcolor=cyan,
%}

%\urlstyle{same}



%%%%%
\usepackage{amsfonts}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

%%%%%%%%%%%%%%%%%% fancy notation command
\newcommand{\llkh}{ \{\!\!\{ }
\newcommand{\rrkh}{ \}\!\!\} }
%%%%%%%%%%%%%%%%%%
%
\newcommand{\VhK}{\mathbb{V}_h^k}
\newcommand{\bxi}{\boldsymbol{\xi}}
%
%\newtheorem{theorem}{Theorem}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{remark}[theorem]{Remark}
%
\newcommand{\ExampleHeatEqn}{Example 5.1}
\newcommand{\ExampleAnisoDiff}{Example 5.2}
\newcommand{\ExamplePorousManuf}{Example 5.3}
\newcommand{\ExamplePorousSmooth}{Example 5.4}
\newcommand{\ExamplePorousDiscontin}{Example 5.5}
\newcommand{\ExampleBlwp}{Example 5.6}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{A generalized framework for DDG methods}{M. E. Danis and J. Yan}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{A generalized framework for direct discontinuous Galerkin methods for nonlinear diffusion equations}%\thanks{Preprint}}
%\funding{Research work of the author is supported by National Science Foundation grant DMS-1620335 and Simons Foundation grant 637716.}}}

% Authors: full names plus addresses.
\author{Mustafa E. Danis\footnotemark[2] \thanks{Department of Aerospace Engineering, Iowa State University, Ames, 50011, USA (\email{danis@iastate.edu}).}
\thanks{asd} \and Jue Yan\thanks{Department of Mathematics, Iowa State University, Ames, 50011, USA (\email{jyan@iastate.edu}).}}
%\thanks{Department of Aerospace Engineering, Iowa State University, Ames, 50011, USA} 
\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

